Faithful to the Document or to the World? Mitigating Hallucinations via Entity-linked Knowledge in Abstractive Summarization

Despite recent advances in abstractive summarization, current summarization systems still suffer from content hallucinations where models generate text that is either irrelevant or contradictory to the source document. However, prior work has been predicated on the assumption that any generated facts not appearing explicitly in the source are undesired hallucinations. Methods have been proposed to address this scenario by ultimately improving `faithfulness' to the source document, but in reality, there is a large portion of entities in the gold reference targets that are not directly in the source. In this work, we show that these entities are not aberrations, but they instead require utilizing external world knowledge to infer reasoning paths from entities in the source. We show that by utilizing an external knowledge base, we can improve the faithfulness of summaries without simply making them more extractive, and additionally, we show that external knowledge bases linked from the source can benefit the factuality of generated summaries.

==> miscs.tex <==
% # 8786 records has been saved to /cns/tp-d/home/octamarine/public/datasets/cnndm/film/val_fae_location_ext_1024.tfr
% # 523 records has been saved to /cns/tp-d/home/octamarine/public/datasets/cnndm/film/val_fae_location_abs_1024.tfr

% # 4886 records has been saved to /cns/tp-d/home/octamarine/public/datasets/xsum/film/test_fae_ext.tfr
% # 3719 records has been saved to /cns/tp-d/home/octamarine/public/datasets/xsum/film/test_fae_abs.tfr

% # 4611 records has been saved to /cns/tp-d/home/octamarine/public/datasets/xsum/film/validation_fae_ext.tfr
% # 3865 records has been saved to /cns/tp-d/home/octamarine/public/datasets/xsum/film/validation_fae_abs.tfr

% # 9746 records has been saved to /cns/tp-d/home/octamarine/public/datasets/xsum/film/test_kafqa.tfr
% # 9800(9786) records has been saved to /cns/tp-d/home/octamarine/public/datasets/xsum/film/validation_kafqa.tfr
% # 177754 records has been saved to /cns/tp-d/home/octamarine/public/datasets/xsum/film/train_kafqa.tfr
% # print(record.document)


% 791 records has been saved to /cns/tp-d/home/octamarine/public/datasets/xsum/film/0_611_validation_fae_512_t5_ext_organization_with_org.tfr
% 791

% 603 records has been saved to /cns/tp-d/home/octamarine/public/datasets/xsum/film/0_473_validation_fae_512_t5_abs_organization_with_org.tfr
% 603

% discuss the problem, not completely solving it. identify the problem

% mixed results?

% factual consistency 
% three cases studies
% (bart results first)
% some analysis of facts 
% missing information and entities. pulling it thgouht knowledge base 

% table 4, most startforward way to appending it

% what if we have the fae and this setting does well .



% \begin{table}[]
% % \hspace{-1cm}
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{l|lll|ll}
% \hline
%  & Abs & Ext & Full & R1 & FCC \\ 
% \toprule
% & & XSUM  &\\
% \midrule
%  T5 & 73.85 & 73.40 & 73.02 & 45.14 & 22.84\\
%  + T5m & \textbf{74.21} & \textbf{73.81} &\textbf{73.48}  & 45.21 & 21.32\\
%  + FaE & 73.15 & 73.21 & 72.74  & 45.09 & 21.32\\
% \midrule
% & & CNN-DM  &\\
% \midrule
%  T5 & 84.12 & 94.26 & 66.85  & 44.32 & 69.22 \\
%  + T5m & \textbf{85.31} & \textbf{96.58} & \textbf{67.15}  & 44.67 & 71.02 \\
%  + FaE & 83.57 & 93.97 & 66.71  & 43.81 & 68.51 \\
% \end{tabular}
% }
% \caption{Results of using FaE for error correction on t5 outputs on XSUM. Metrics that capture Consistency only.}
% \label{tab:main_results_consistency}
% \end{table}



% \begin{table}[]
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}[\columnwidth]{l|llllll}
% \toprule
%             & wo. f. &  wo. f.  &  w. f. &  w. f. & in & in \\ \midrule
%              & ext  & abs  & ext & abs  & src & KB \\ \midrule
% location     & 0.95      & 0.75 & 0.95      & 0.7  & 40\%      & 19\%  \\ 
% person       & 0.75      & 0.60 & 0.75      & 0.65 & 29\%      & 8\%   \\ 
% event        & 0.62      & 0.40 & 0.62      & 0.35 & 21\%      & 12\%  \\ 
% other        & 0.25      & 0.30 & 0.25      & 0.30 & 34\%      & 7\%   \\ 
% organization & 0.50      & 0.50 & 0.50      & 0.40 & 40\%      & 13\%  \\ 
% art          & 0.59      & 0.14 & 0.59      & 0.14 & 32\%      & 15\%  \\ \bottomrule
% \end{tabular}
% }
%  \caption{Results of fact expert correction accuracy by categories.}
%   \label{tab:result_categories}
% \end{table}

% c-after,c-before, c-good, c-bad, c-n\\
% (25, 23, 21, 29, 1)\\
% (29, 23, 14, 33, 0)\\
% (24, 26, 18, 31, 0)\\

% kappa 0.7391646182060404
% fleiss 0.7391150442477875
% alpha 0.7396555345515647
% scotts 0.7387759924385632
